Exploring Diffusion Models for Unsupervised Video Anomaly Detection

This paper investigates the performance of diffusion models for video anomaly detection (VAD) within the most challenging but also the most operational scenario in which the data annotations are not used. As being sparse, diverse, contextual, and often ambiguous, detecting abnormal events precisely is a very ambitious task. To this end, we rely only on the information-rich spatio-temporal data, and the reconstruction power of the diffusion models such that a high reconstruction error is utilized to decide the abnormality. Experiments performed on two large-scale video anomaly detection datasets demonstrate the consistent improvement of the proposed method over the state-of-the-art generative models while in some cases our method achieves better scores than the more complex models. This is the first study using a diffusion model and examining its parameters' influence to present guidance for VAD in surveillance scenarios.

==> ref_fullName.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@inproceedings{Karras2022edm,
  author    = {Tero Karras and Miika Aittala and Timo Aila and Samuli Laine},
  title     = {Elucidating the Design Space of Diffusion-Based Generative Models},
  booktitle = {Proc. NeurIPS},
  year      = {2022}
}

@inproceedings{ren2021deep,
  title={Deep video anomaly detection: Opportunities and challenges},
  author={Ren, Jing and Xia, Feng and Liu, Yemeng and Lee, Ivan},
  booktitle={2021 international conference on data mining workshops (ICDMW)},
  pages={959--966},
  year={2021},
  organization={IEEE}
}

@inproceedings{luo2017revisit,
  title={A revisit of sparse coding based anomaly detection in stacked rnn framework},
  author={Luo, Weixin and Liu, Wen and Gao, Shenghua},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={341--349},
  year={2017}
}

@inproceedings{ravanbakhsh2017abnormal,
  title={Abnormal event detection in videos using generative adversarial nets},
  author={Ravanbakhsh, Mahdyar and Nabi, Moin and Sangineto, Enver and Marcenaro, Lucio and Regazzoni, Carlo and Sebe, Nicu},
  booktitle={2017 IEEE international conference on image processing (ICIP)},
  pages={1577--1581},
  year={2017},
  organization={IEEE}
}

@article{sabokrou2017deep,
  title={Deep-cascade: Cascading 3d deep neural networks for fast anomaly detection and localization in crowded scenes},
  author={Sabokrou, Mohammad and Fayyaz, Mohsen and Fathy, Mahmood and Klette, Reinhard},
  journal={IEEE Transactions on Image Processing},
  volume={26},
  number={4},
  pages={1992--2004},
  year={2017},
  publisher={IEEE}
}

@inproceedings{smeureanu2017deep,
  title={Deep appearance features for abnormal behavior detection in video},
  author={Smeureanu, Sorina and Ionescu, Radu Tudor and Popescu, Marius and Alexe, Bogdan},
  booktitle={Image Analysis and Processing-ICIAP 2017: 19th International Conference, Catania, Italy, September 11-15, 2017, Proceedings, Part II 19},
  pages={779--789},
  year={2017},
  organization={Springer}
}

@article{zhang2016video,
  title={Video anomaly detection based on locality sensitive hashing filters},
  author={Zhang, Ying and Lu, Huchuan and Zhang, Lihe and Ruan, Xiang and Sakai, Shun},
  journal={Pattern Recognition},
  volume={59},
  pages={302--311},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{zaheer2020old,
  title={Old is gold: Redefining the adversarially learned one-class classifier training paradigm},
  author={Zaheer, Muhammad Zaigham and Lee, Jin-ha and Astrid, Marcella and Lee, Seung-Ik},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14183--14193},
  year={2020}
}

@article{chandola2009anomaly,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys (CSUR)},
  volume={41},
  number={3},
  pages={1--58},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gong2019memorizing,
  title={Memorizing normality to detect anomaly: Memory-augmented deep autoencoder for unsupervised anomaly detection},
  author={Gong, Dong and Liu, Lingqiao and Le, Vuong and Saha, Budhaditya and Mansour, Moussa Reda and Venkatesh, Svetha and Hengel, Anton van den},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1705--1714},
  year={2019}
}

@article{mohammadi2021image,
  title={Image/video deep anomaly detection: A survey},
  author={Mohammadi, Bahram and Fathy, Mahmood and Sabokrou, Mohammad},
  journal={arXiv preprint arXiv:2103.01739},
  year={2021}
}

@inproceedings{majhi2021dam,
  title={DAM: Dissimilarity Attention Module for Weakly-supervised Video Anomaly Detection},
  author={Majhi, Snehashis and Das, Srijan and Br{\'e}mond, Fran{\c{c}}ois},
  booktitle={2021 17th IEEE International Conference on Advanced Video and Signal Based Surveillance (AVSS)},
  pages={1--8},
  year={2021},
  organization={IEEE}
}

@inproceedings{tian2021weakly,
  title={Weakly-supervised video anomaly detection with robust temporal feature magnitude learning},
  author={Tian, Yu and Pang, Guansong and Chen, Yuanhong and Singh, Rajvinder and Verjans, Johan W and Carneiro, Gustavo},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={4975--4986},
  year={2021}
}

@inproceedings{zaheer2020claws,
  title={Claws: Clustering assisted weakly supervised learning with normalcy suppression for anomalous event detection},
  author={Zaheer, Muhammad Zaigham and Mahmood, Arif and Astrid, Marcella and Lee, Seung-Ik},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XXII 16},
  pages={358--376},
  year={2020},
  organization={Springer}
}

@inproceedings{zhang2019temporal,
  title={Temporal convolutional network with complementary inner bag loss for weakly supervised anomaly detection},
  author={Zhang, Jiangong and Qing, Laiyun and Miao, Jun},
  booktitle={2019 IEEE International Conference on Image Processing (ICIP)},
  pages={4030--4034},
  year={2019},
  organization={IEEE}
}

@inproceedings{zaheer2022generative,
  title={Generative cooperative learning for unsupervised video anomaly detection},
  author={Zaheer, M Zaigham and Mahmood, Arif and Khan, M Haris and Segu, Mattia and Yu, Fisher and Lee, Seung-Ik},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14744--14754},
  year={2022}
}

@article{kim2021semi,
  title={Semi-orthogonal embedding for efficient unsupervised anomaly segmentation},
  author={Kim, Jin-Hwa and Kim, Do-Hyeong and Yi, Saehoon and Lee, Taehoon},
  journal={arXiv preprint arXiv:2105.14737},
  year={2021}
}

@inproceedings{park2020learning,
  title={Learning memory-guided normality for anomaly detection},
  author={Park, Hyunjong and Noh, Jongyoun and Ham, Bumsub},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={14372--14381},
  year={2020}
}

@article{zaheer2022stabilizing,
  title={Stabilizing adversarially learned one-class novelty detection using pseudo anomalies},
  author={Zaheer, Muhammad Zaigham and Lee, Jin-Ha and Mahmood, Arif and Astrid, Marcella and Lee, Seung-Ik},
  journal={IEEE Transactions on Image Processing},
  volume={31},
  pages={5963--5975},
  year={2022},
  publisher={IEEE}
}


@InProceedings{Schneider_2022_CVPR,
    author    = {Schneider, Pascal and Rambach, Jason and Mirbach, Bruno and Stricker, Didier},
    title     = {Unsupervised Anomaly Detection From Time-of-Flight Depth Images},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
    month     = {June},
    year      = {2022},
    pages     = {231-240}
}


@inproceedings{li2021unsupervised,
  title={Unsupervised Video Anomaly Detection Based on Sparse Reconstruction},
  author={Li, ZhenJiang and Yang, Wenbo and Wu, Guangli and Liu, Liping},
  booktitle={Big Data Analytics for Cyber-Physical System in Smart City: BDCPS 2020, 28-29 December 2020, Shanghai, China},
  pages={994--1001},
  year={2021},
  organization={Springer}
}

@inproceedings{sultani2018real,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={6479--6488},
  year={2018}
}

@INPROCEEDINGS{liu2018ano_pred, 
        author={W. Liu and W. Luo, D. Lian and S. Gao}, 
        booktitle={2018 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
        title={Future Frame Prediction for Anomaly Detection -- A New Baseline}, 
        year={2018} 
}
